Fast, Diverse and Accurate Image Captioning Guided By Part-of-Speech

Image captioning is an ambiguous problem, with many suitable captions for an image. To address ambiguity, beam search is the de facto method for sampling multiple captions. However, beam search is computationally expensive and known to produce generic captions. To address this concern, some variational auto-encoder (VAE) and generative adversarial net (GAN) based methods have been proposed. Though diverse, GAN and VAE are less accurate. In this paper, we first predict a meaningful summary of the image, then generate the caption based on that summary. We use part-of-speech as summaries, since our summary should drive caption generation. We achieve the trifecta: (1) High accuracy for the diverse captions as evaluated by standard captioning metrics and user studies; (2) Faster computation of diverse captions compared to beam search and diverse beam search; and (3) High diversity as evaluated by counting novel sentences, distinct n-grams and mutual overlap (i.e., mBleu-4) scores.

==> intro.tex <==
% !TEX root = divcap.tex
\section{Introduction}


Image captioning entails generating a realistic description for a 
given image. It is applicable across domains from 
robotics and virtual assistants to  tools for the visually
impaired. A large body of literature has focused on developing predictive image captioning techniques, often using recurrent 
neural nets (RNN)~\cite{Mao2014DeepCW,show_tell,show_attend_tell,neuraltalk,Panderson}. 
More recently~\cite{AnejaConvImgCap17,Wang2018CNNCNNCD}, demonstrate 
predictive captioning with accuracies similar to RNNs while using convolutional networks. 

However, image captioning is also an ambiguous problem, \ie, there is more than one sentence
that can appropriately describe an image. Therefore, methods that can 
generate multiple and diverse image captions are important. 
But machine generated diverse captions have not reached the quality of 
human generated ones. Generally, the diversity and nuances present in captions 
written by different humans are absent in  diverse captions generated 
by current deep net models. In this paper, we address the task of 
diverse image captioning.

\begin{table}[!t]
\vspace{-.3cm}
\begin{center}
\begin{tabular}{l|ccc}
\toprule
	Method & Fast & Diverse  & Accurate \\
\toprule
	Beam search & $\times$ & $\times$ & \checkmark \\
	Diverse beam search~\cite{VijayakumarCSSL18} & $\times$ & $\times$ & \checkmark \\
	AG-CVAE~\cite{WangVAECaption} & - & $\checkmark$ & $\times$ \\
	Ours (POS) &  \checkmark &  \checkmark &  \checkmark \\
\toprule
\end{tabular}
\vspace{-.3cm}
	\caption{We show that our part-of-speech (POS) based method achieves the trifecta
		of {\bf high accuracy, fast computation} and {\bf more diversity}. Beam search and 
		diverse beam search are slow. They also produce captions with high mutual
		overlap and lower distinct $n$-grams than POS (see mBleu-4, div-1 and 
		div-2 in \tabref{tab:diversity}). POS outperforms AG-CVAE on captioning
		metrics in \figref{fig:topk} and is therefore  more accurate.
		{\color{blue}why is there a dash for AG-CVAE?}
		}
\vspace{-1cm}
\label{tab:summary}
\end{center}
\end{table}




Beam search is the classical method to sample multiple solutions given 
 sequence models for neural machine translation and image captioning. 
However, beam search with wide beams is very slow. This limits the 
number of captions that can be sampled with beam search. Moreover, beam search
is also known to generate generic captions that lack diversity~\cite{Finkel2006,Gimpel13asystematic}. 
To address this concern, variational auto-encoder (VAE)~\cite{WangVAECaption} and generative 
adversarial net (GAN) formulations~\cite{DaiICCV17,shetty2017speaking,li2018generating} 
have been proposed, which %. VAE and GAN-based methods 
outperform beam search on 
diversity metrics. VAE and GAN-based methods   rely on sampling latent vectors from a 
learned or a simple, \eg, uniform distribution. Then, they generate multiple captions 
conditioned on these sampled latent vectors. However, these latent 
vectors are not grounded in any semantic image or language priors. 
This makes the captions less accurate compared to beam search. For
example, in Tab.\ 1 of~\cite{shetty2017speaking}, beam search shows higher accuracy on captioning metrics than 
GAN results. 

In this paper, we replace this abstract latent space with a semantic latent space 
conditioned on a part-of-speech  (POS)  tag sequence. 
%For captioning, classical methods condition each 
%word on the image and all previous words in a sentence. 
Hence, in this work, beyond conditioning of generation on the image and all previous words in a generated sentence, we additionally 
condition on a POS tag sequence. This offers the inference procedure an approximate 
global view of the sentence being generated at each step. It can then generate a caption that 
adheres roughly to this global view. Sampling different POS tag 
sequences permits to generate multiple captions. Our procedure produces diverse 
sentences because sentences that adhere to different tag sequences have meaningful 
diversity.  
Our main contributions are twofold: 
\begin{itemize}[itemsep=0pt,leftmargin=0in]
  \item[] {\bf Incorporate natural language prior.} Our POS captioning network incorporates 
	  POS tag sequences as a natural language prior (see \secref{sec:poscap}). 
	  We demonstrate that this prior can be inferred from the image (see \secref{sec:posclassify}). 
	  %In future, our techniques can be extended to other tasks with different 
	  %output spaces and corresponding priors.
  \item[] {\bf Develop fast, accurate and diverse sampling method for captions.} We show that image
	  captioning with POS tag sequences is fast, diverse and accurate. Our POS 
	  methods sample captions faster and with more diversity than techniques based on beam 
	  search and its variant diverse beam search~\cite{VijayakumarCSSL18}. Our 
	  diverse captions are more accurate than their counterparts produced by GANs~\cite{shetty2017speaking} 
	  (\tabref{tab:gan}) and VAEs~\cite{WangVAECaption} (\tabref{tab:consensus}, 
	  \figref{fig:topk}). \tabref{tab:summary} summarizes our results discussed in detail in 
	  Sections~\ref{sec:top1} to~\ref{sec:speed} and compares different methods in terms of speed, diversity 
	  and accuracy. 
\end{itemize}

The paper is organized as follows. \secref{sec:relwork} discusses relevant related
work. Our notation and the classical approach to image captioning is discussed in
\secref{sec:background}. We present our captioning approach conditioned on part-of-speech 
in \secref{sec:poscap}. Finally, \secref{sec:res} provides our experimental results. 

{\color{blue}I would show a teaser Fig instead of the table on page 1}

%Our results show a significant improvement on 
%captioning metrics for our generated captions (See \secref{sec:top1} and \ref{sec:topk}). 
%Thus, our method does {\it efficient and accurate} search for the modes in the caption 
%space.  

%\begin{figure}[!t]
%\centering
%\includegraphics[width=.9\textwidth,trim={0cm 1.3cm 0cm 2cm},clip]{fig/posfig.pdf}
%\vspace{-.25cm}
%\caption{Our caption conditions on some of the characteristics of part-of-speech (POS). 
%We can add adjectives (e.g. grassy; red and yellow), modify noun phrases (e.g. cheese 
%and vegetables), add numerical qualifiers (e.g. two) with appropriate POS tags. 
%This conditioning is highlighted in blue/green colors. See \secref{sec:background} 
%for details of POS tags. Note, due to quantization (See \secref{sec:posquant}) the 
%generated caption may not exactly adhere to the POS tag sequence.}
%\vspace{-.6cm}
%\label{fig:editpos}
%\end{figure}


%\begin{figure}
%\centering
%\includegraphics[width=.8\textwidth,trim={2cm 7cm 2cm 2cm},clip]{fig/teaser.pdf}
%\caption{We show 4 diverse captions produced by our parts of speech (POS) captioning method. The distinctive parts of each caption are marked in color.}
%\label{fig:teaser}
%\end{figure}

%Notable advances have been 
%made in conditioning image captioning on semantic prior of objects via 
%use of object detectors~\cite{Lu2018Neural,WangObjectCounts}. This conditioning or control 
%is only limited to the objects (or nouns) in the caption and ignores the remainder. 

%To obtain multiple captions, Beam Search (BS) can be used on  word-wise posterior probabilities generated by 
%CNNs/RNNs~\cite{show_tell,neuraltalk}. BS maintains top-$k$ (incomplete) 
%captions ordered by likelihood and expands top-$k$ captions greedily from 
%start to end of sentence. However, BS is computationally inefficient for 
%large beam size (i.e., large $k$) and known to lack 
%diversity~\cite{LiGBGD16,VijayakumarCSSL18}. Therefore, there is a need for 
%effective and efficient sampling mechanisms that take into account the 
%ambiguity of image captioning. 

%Our proposed approach is able to construct
%diverse sentences that follow the part-of-speech guidance.
%We evaluate our proposed approach on the challenging MS-COCO dataset~\cite{},
%showing {\color{blue}xxx}. Qualitative results of the proposed approach are
%illustrated in \figref{fig:teaser}. Going forward we envision part-of-speech
%guidance to be particularly useful for paragraph generation.

%Those methods leverage the
%fact that a metric comparing textual descriptions and images can be learned.
%While those approaches work well for a small number of textual descriptions,
%computational challenges arise once we consider a reasonably large set of
%possible captions. Moreover, it seems hard to construct a reasonably
%small set of captions that describe any possible scene sufficiently
%accurately.

%\begin{figure}[t] \centering \includegraphics[width=5cm]{fig/kaw.png}
%\caption{Part-of-speech guided captions, generated with our approach}
%\label{fig:teaser} \end{figure}



